Reinforced Genetic Algorithm for Structure-based Drug Design

Structure-based drug design (SBDD) aims to discover drug candidates by finding molecules (ligands) that bind tightly to a disease-related protein (targets), which is the primary approach to computer-aided drug discovery. Recently, applying deep generative models for three-dimensional (3D) molecular design conditioned on protein pockets to solve SBDD has attracted much attention, but their formulation as probabilistic modeling often leads to unsatisfactory optimization performance. On the other hand, traditional combinatorial optimization methods such as genetic algorithms (GA) have demonstrated state-of-the-art performance in various molecular optimization tasks. However, they do not utilize protein target structure to inform design steps but rely on a random-walk-like exploration, which leads to unstable performance and no knowledge transfer between different tasks despite the similar binding physics. To achieve a more stable and efficient SBDD, we propose Reinforced Genetic Algorithm (RGA) that uses neural models to prioritize the profitable design steps and suppress random-walk behavior. The neural models take the 3D structure of the targets and ligands as inputs and are pre-trained using native complex structures to utilize the knowledge of the shared binding physics from different targets and then fine-tuned during optimization. We conduct thorough empirical studies on optimizing binding affinity to various disease targets and show that RGA outperforms the baselines in terms of docking scores and is more robust to random initializations. The ablation study also indicates that the training on different targets helps improve performance by leveraging the shared underlying physics of the binding processes. The code is available at https://github.com/futianfan/reinforced-genetic-algorithm.

==> NeurIPS 2022 RGA arxiv/experiment.tex <==
\section{Experiment}
\label{sec:experiment}

In this section, we briefly describe the experimental setup and results. The Appendix includes more details, including software configuration, implementation details, dataset description \& processing, hyperparameter tuning, ablation study, and additional experimental results. 
The code is available at \url{https://github.com/futianfan/reinforced-genetic-algorithm}. 



\subsection{Experimental Setup}
\label{sec:setup}


\noindent\textbf{Docking Simulation}. 
We adopt AutoDock Vina~\cite{trott2010autodock} to evaluate the binding affinity. The docking score estimated by AutoDock Vina is called Vina score and roughly characterizes the free energy changes of binding processes in kcal/mol. 
Thus lower Vina score means a stronger binding affinity between the ligand and target. 
%In the implementation, we maximize the negative value of the docking score. 
 We picked various disease-related proteins, including G-protein coupling receptors (GPCRs) and kinases from DUD-E~\cite{mysinger2012directory} and the SARS-CoV-2 main protease~\cite{zhang2021potent} as targets. Please see the Appendix for more information.


\noindent\textbf{Baselines}. 
The baseline methods cover traditional brute-force search methods (Screening), deep generative models (JTVAE and Gen3D), genetic algorithm (GA+D, graph-GA, Autogrow 4.0), reinforcement learning methods (MolDQN, RationaleRL, REINVENT, GEGL), and MCMC method (MARS).
Gen3D and Autogrow 4.0 are structure-based drug design methods, while others are general-purpose molecular design methods.
Although methods explicitly utilizing target structures are relatively few, we add general-purpose molecular design methods optimizing the same docking oracle scores as ours, which is a common use case, as baselines~\cite{jensen2019graph,huang2021therapeutics}. 
Concretely, 
\textbf{Screening} mimics high throughput screening via sampling from ZINC database randomly; 
\textbf{JTVAE} (Junction Tree Variational Auto-Encoder)~\cite{jin2018junction} uses a Bayesian optimization on the latent space to indirectly optimize molecules; 
\textbf{Gen3D}~\cite{luo20213d} is an auto-regressive generative model that grows 3D structures atom-wise inside the binding pocket; 
\textbf{GA+D}~\cite{nigam2019augmenting} represents molecule as SELFIES string~\cite{krenn2020self} and uses genetic algorithm enhanced by a discriminator neural network; 
\textbf{Graph-GA}~\cite{jensen2019graph} conduct genetic algorithm on molecular graph representation;   
\textbf{Autogrow 4.0}~\cite{spiegel2020autogrow4} is the state-of-the-art genetic algorithm in structure-based drug design;
\textbf{MolDQN} (Molecule Deep Q-Network)~\cite{zhou2019optimization}  leverages deep Q-value learning to grow molecules atom-wisely; 
\textbf{RationaleRL}~\cite{jin2020multi} uses rationale (e.g., functional groups or subgraphs) as the building block and a policy gradient method to guide the training of graph neural network-based generator; 
\textbf{REINVENT}~\cite{Olivecrona} represent molecules as SMILES string and uses policy gradient based reinforcement learning methods to guide the training of the RNN generator; 
 \textbf{GEGL} (genetic expert-guided learning)~\cite{ahn2020guiding} uses LSTM guided by reinforcement learning to imitate the GA exploration; 
\textbf{MARS} (Markov Molecule Sampling)~\cite{xie2021mars} leverages Markov chain Monte Carlo sampling (MCMC) with adaptive proposal and annealing scheme to search chemical space.
% \textbf{GCPN} (Graph Convolutional Policy Network)~\cite{You2018-xh}; 
To conduct a fair comparison, we limit the number of oracle calls to 1,000 times for each method. 
All the baselines can be run with one-line code using the software (\url{https://github.com/wenhao-gao/mol_opt}) in practical molecular optimization benchmark~\cite{gao2022sample}. 
% Implementation details of all the baseline methods are available in Appendix. 

\noindent\textbf{Dataset}: we randomly select molecules from ZINC~\cite{sterling2015zinc} database (around 250 thousands drug-like molecules) as 0-th generation of the genetic algorithms (\mname, Autogrow 4.0, GA+D). ZINC also serves as the training data for pretraining the model in JTVAE, REINVENT, RationaleRL, etc. We adopt {CrossDocked2020}~\cite{francoeur2020three} dataset that contains around 22 million ligand-protein complexes as the training data for pretraining the policy neural networks, as mentioned in Section~\ref{sec:policy_net}. More descriptions are available in Appendix. 

\noindent\textbf{Metrics}. 
The selection of evaluation metrics follows recent works in molecule optimization~\cite{jin2018junction,nigam2019augmenting,jin2020multi,xie2021mars} and \marked{structure}-based drug design~\cite{spiegel2020autogrow4,luo20213d,huang2021therapeutics}. 
For each method, we select top-100 molecules with the best docking scores for evaluation and consider the following metrics: 
{\textbf{TOP-1/10/100} (average docking score of top-1/10/100 molecules)}: docking score directly measures the binding affinity between the ligand and target and is the most informative metric in structure-based drug design; 
\textbf{Novelty (Nov)} {(\% of the generated molecules that are not in training set)}; 
\textbf{Diversity (Div)} {(average pairwise Tanimoto distance between the Morgan fingerprints)}; 
We also evaluate some simple {pharmaceutical properties}, including quantitative drug-likeness (\textbf{QED}) and synthetic accessibility (\textbf{SA}). QED score indicates drug-likeliness ranging from 0 to 1 (higher the better). SA score ranges from 1 to 10 (lower the better). All the evaluation functions are available at Therapeutics data commons (TDC, \url{https://tdcommons.ai/fct_overview})~\cite{huang2021therapeutics,Huang2022artificial}. 


% \noindent\textbf{Metrics}. 
% The selection of evaluation metrics follows recent works in molecule optimization~\cite{jin2018junction,nigam2019augmenting,jin2020multi,xie2021mars} and structure-based drug design~\cite{spiegel2020autogrow4,luo20213d,huang2021therapeutics}. 
% For each method, we select top-100 molecules with best docking scores for evaluation, and consider the following metrics: 
% {\textbf{TOP-1/10/100} (average docking score of top-1/10/100 molecules)}: docking score directly measures the binding affinity between the ligand and target and is the most informative metric in structure based drug design; 
% \textbf{Novelty (Nov)} {(\% of the generated molecules that are not in training set)}; 
% \textbf{Diversity (Div)} {(average pairwise Tanimoto distance between the Morgan fingerprints)}; 
% % (4) \textbf{\# of oracle calls}: the number of oracle call measures the sample efficiency of a method. For each method, we set the number of oracle calls so that the docking score nearly converge w.r.t. oracle call’s number. 
% % Since we only enumerate valid chemical structures during the recovery from scaffolding trees (Section~\ref{sec:assemble}), the chemical validities are always 100\%. 
% % Details are in Section~\ref{sec:metrics}. 
% We also evaluate some simple {molecular pharmaceutical properties}, including quantitative drug-likeness (\textbf{QED}) and synthetic accessibility (\textbf{SA}). QED score is an indicator of drug-likeness ranging from 0 to 1, higher QED score is more desirable. SA scores ranges from 0 to infinity, lower SA score represents better synthetic accessibility~\cite{gao2020synthesizability}. 






\subsection{Results}
\label{sec:results}


\begin{table*}[t!]
\centering
\vspace{-15pt}
\caption{The summarized performance of different methods. The mean and standard deviation across targets are reported. 
Arrows ($\uparrow$, $\downarrow$) indicate the direction of better performance. 
% Screening searches over the existing drug database, ZINC, so the novelty is 0.0\%. 
For each metric, the best method is underlined and the top-3 methods are bolded. 
\mname -pretrain and \mname -KT are two variants of \mname that without pretraining and without training on different target proteins, respectively.
% more discussions are in ``Knowledge trasfer between protein targets'' in Section~\ref{sec:results}. 
}
\label{table:result}
 \resizebox{0.98\textwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule[0.6pt]
Method & TOP-100$\downarrow$ & TOP-10$\downarrow$ & TOP-1$\downarrow$ & Nov$\uparrow$ & Div$\uparrow$ & QED$\uparrow$ &  SA$\downarrow$  \\
\hline 
screening & -9.351\std{0.643} & -10.433\std{0.563} & -11.400\std{0.630} & 0.0\std{0.0}\% & 0.858\std{0.005} & 0.678\std{0.022} & 2.689\std{0.077} \\ 
MARS & -7.758\std{0.612} & -8.875\std{0.711} & -9.257\std{0.791} & 100.0\std{0.0}\% & {\bf\underline{0.877\std{0.001}}} &  {\bf 0.709\std{0.008}} & {\bf\underline{2.450\std{0.034}}} \\  
MolDQN & -6.287\std{0.396} & -7.043\std{0.487} & -7.501\std{0.402} & 100.0\std{0.0}\% & {\bf 0.877\std{0.009}} & 0.170\std{0.024} & 5.833\std{0.182}  \\ 
% \tabdashline 
GEGL & -9.064\std{0.920} & -9.91\std{0.990} & -10.45\std{1.040} & 100.0\std{0.0}\% & 0.853\std{0.003} & 0.643\std{0.014} & 2.99\std{0.054} \\ 
REINVENT & { -10.181\std{0.441}} & { -11.234\std{0.632}} & { -12.010\std{0.833}} & 100.0\std{0.0}\% & 0.857\std{0.011} &  0.445\std{0.058} & 2.596\std{0.116}  \\
RationaleRL & -9.233\std{0.920} & -10.834\std{0.856} & -11.642\std{1.102} & 100.0\std{0.0}\% & 0.717\std{0.025} & 0.315\std{0.023} & 2.919\std{0.126} \\ 
JTVAE & -9.291\std{0.702} & -10.242\std{0.839} & -10.963\std{1.133} & 98.0\std{0.027}\% &  0.867\std{0.001} & 0.593\std{0.035} & 3.222\std{0.136} \\ 
Gen3D & -8.686\std{0.450} & -9.285\std{0.584} & -9.832\std{0.324} & 100.0\std{0.0}\% & {\bf 0.870\std{0.006}} & 0.701\std{0.016} & 3.450\std{0.120} \\ 
GA+D & -7.487\std{0.757} & -8.305\std{0.803} & -8.760\std{0.796} & 99.2\std{0.011}\%  & 0.834\std{0.035} & 0.405\std{0.024} & 5.024\std{0.164} \\ 
Graph-GA & {\bf -10.848\std{0.860}} & {\bf -11.702\std{0.930}} & {\bf -12.302\std{1.010}} & 100.0\std{0.0}\% &  0.811\std{0.037} & 0.456\std{0.067} & 3.503\std{0.367} \\ 
Autogrow 4.0 & {\bf -11.371\std{0.398}} & {\bf -12.213\std{0.623}} & {\bf -12.474\std{0.839}} & 100.0\std{0.0}\% & 0.852\std{0.011} & {\bf 0.748\std{0.022}} & {\bf{2.497\std{0.049}}} \\ 
RGA (ours) & {\bf\underline{-11.867\std{0.170}}} & \underline{\bf{-12.564\std{0.287}}} & {\bf\underline{-12.869\std{0.473}}} & 100.0\std{0.0}\% & 0.857\std{0.020} & {\bf\underline{ 0.742\std{0.036}}} & {\bf 2.473\std{0.048}}  \\ \toprule 
RGA - pretrain & -11.443\std{0.219} & -12.424\std{0.386} & -12.435\std{0.654} & 100.0\std{0.0}\% & 0.854\std{0.035} & 0.750\std{0.034} & 2.494\std{0.043} \\ 
RGA - KT & -11.434\std{0.169} & -12.437\std{0.354} & -12.502\std{0.603} & 100.0\std{0.0}\% & 0.853\std{0.028} & 0.738\std{0.034} & 2.501\std{0.050} \\ 
\bottomrule[0.6pt]
\end{tabular}}
\end{table*}

\noindent\textbf{Stronger Optimization Performance}. 
We summarized the main results of the structure-based drug design in Table~\ref{table:result}. 
We evaluate all the methods on all targets and report each metric's mean and standard deviations across all targets. 
Our result shows \mname achieves the best performance in TOP-100/10/1 scores among all methods we compared. 
Compared to Autogrow 4.0, \mname's better performance in docking score demonstrates that the policy networks contribute positively to the chemical space navigation and eventually help discover more potent binding molecules.
On the other hand, including longer-range navigation steps enabled by crossover leads to superior performance than other RL methods  (REINVENT, MolDQN, GEGL and RationaleRL) that only focus on local modifications. In addition, we also observed competitive structure quality measured by QED ($>0.7$) and SA\_Score ($<2.5$) in Autogrow 4.0 and \mname without involving them as optimization objectives, thanks to the mutation steps originating from chemical reactions. We visualize two designed ligands with optimal affinity for closer inspection in Figure~\ref{fig:7l11} and~\ref{fig:3eml}, and find both ligands bind tightly with the targets. 

% \noindent\textbf{Stronger Optimization Performance}. The main results of structure based drug design are reported in Table~\ref{table:result}. We evaluate all the methods across different targets and report the mean results and their standard deviations. 
% We have the following key observations: 
% (i) Autogrow 4.0 achieves best docking scores in terms of TOP-100/10/1 scores among all the compared baseline methods and are also competitive in other metrics. This validates the superiority of assemble strategy and well-crafted crossover/mutation operations in Autogrow 4.0. 
% (ii) RGA outperforms autogrow 4.0 consistently on docking score, achieving around 0.5, 0.3 and 0.4 absolute improvement in terms of average TOP-100/10/1 docking scores, respectively (-11.867 vs -11.371, -12.564 vs -12.213, -12.869 vs -12.474). The improvement attributes to more sophisticated navigation scheme brought by RL (compared with random selection in Autogrow 4.0). 
% (iii) RGA obtains significant improvement compared with other reinforcement learning methods (REINVENT, MolDQN and rationaleRL), reaching 16.6\%, 88.7\% and 28.5\% improvement over REINVENT, MolDQN and rationaleRL respectively (-10.181 vs -11.867, -6.287 vs 11.867, -9.233 vs 11.867) in terms of TOP-100 docking score (the most important metric). This indicates the importance of assemble strategy in optimization performance. 
% (iv) Almost all the methods (except screening) achieve nearly 100\% novelty, validating the strong ability of generation methods that generate new molecules that does not appear in training data; screening searches over ZINC, the exising drug database, thus its novelty is zero. 
% All the methods except RationaleRL exhibit higher diversity (all values are greater than 0.80) with small variances (all the reported standard deviations are less than 0.05). 
% (v) \mname are also competitive on some basic pharmaceutical properties, including QED and SA score, although these properties are not involved optimization objective. \mname achieve desirable results in terms of QED scores ($>0.7$), indicating the generated molecules are more drug-like; Autogrow 4.0 and \mname are able to generate easily synthesizable molecules, whose average SA scores are less than 2.5. The main reason is the reaction based mutation operations (described in Section~\ref{sec:ga}) enhance the synthesizability of the generated molecule. 
% We visualize examples of the binding sites and their top
% affinity ligands' poses for closer inspection in Figure~\ref{fig:7l11} and~\ref{fig:3eml}. 


\noindent\textbf{Suppressed Random-Walk Behavior}.
Especially in SBDD, when the oracle functions are expensive molecular simulations, robustness to random seeds is essential for improving the worst-case performance of algorithms. One of the major issues in traditional GAs is that they have a significant variance between multiple independent runs as they randomly select parents for crossover and mutation types. To examine this behavior, we run five independent runs for \mname, Autogrow 4.0 and graph-GA (three best baselines, all are GA methods) on all targets and plot the standard deviations between runs in Figure~\ref{fig:randomwalk1} and \ref{fig:randomwalk2}. With policy networks guiding the action steps, we observed that the random-walk behavior in Autogrow 4.0 was suppressed in \mname, indicated by the smaller variance. Especially in the later learning phase (after 500 oracle calls), the policy networks are fine-tuned and guide the search more intelligently. This advantage leads to improved worst-case performance and a higher probability of successfully identifying bioactive drug candidates with constrained resources.

% \noindent\textbf{Suppressed Random-Walk Behavior}. 
% As mentioned, in the traditional GA, the crossover and mutation operation randomly selects the ligands and reactions, this kind of random-walk behavior usually leads to high variance and are undesirable in molecule optimization. 
% \mname is designed to suppress this random-walk behavior. Specifically, we conduct multiple independent runs to compare the \mname and its random-walk version, i.e., Autogrow 4.0. The average TOP-100 and TOP-10 vina score over 5 independent runs, and their standard deviations are reported in Figure~\ref{fig:randomwalk1} and~\ref{fig:randomwalk2}, respectively. We observe that \mname is able to significantly reduce the variance, especially in the later learning phase (after 500 oracle calls). 
% The observation validates \mname's ability to suppress random-walk behavior. 

\noindent\textbf{Knowledge Transfer Between Protein Targets}. 
To verify if \mname benefited from learning the shared physics of ligand-target interaction, we conducted an ablation study whose results are in the last two rows of Table~\ref{table:result}. Specifically, we compare \mname with two variants: (1) \mname-pretrain that does not pretrain the policy network with all native complex structures in the {CrossDocked2020}; (2) \mname-KT (knowledge transfer) that fine-tune the networks with data of individual target independently. We find that both strategies positively contribute to \mname on TOP-100/10/1 docking score. These results demonstrate the policy networks successfully learn the shared physics of ligand-target interactions and leverage the knowledge to improve their performance.


% \noindent\textbf{Knowledge Transfer Between Protein Targets}. 
% \mname is able to learn the knowledge of different protein targets using the ENN based target ligand policy network (Section~\ref{sec:policy_net}), which is pretrained on 3D target-ligand binding affinity prediction
%  task. To explore their empirical effect, we compare \mname with two variants: (1) \mname-pretrain does not pretrain the policy network. (2) \mname-KT (knowledge transfer) does not leverage the knowledge learned from other targets and optimize individual target independently. The results are also reported in the last two rows of Table~\ref{table:result}. We find that both strategies positively contribute to \mname on TOP-100/10/1 docking score. The reason is pretraining learns the 3D target-ligand structure information and provides a warm start for the policy network, knowledge transfer (KT) can learn the pattern of target-ligand binding physics from a large amount of data and promote the optimization performance. 
 
% \noindent\textbf{Case study}
% Also, we visualize examples of the binding sites and their top
% affinity ligands' poses for closer inspection in Figure~\ref{fig:7l11} and~\ref{fig:3eml}. 
% %%Figure~\ref{fig:demo}. 
% We observe that the ligand binds tightly with the target structure. 
% The example validates the ability of \mname to generate the high binding affinity molecules for designated target. 












\begin{figure}[t!]
\centering
\vspace{-15pt}
\subfigure[Example of 7l11, -10.8 kcal/mol]{
\includegraphics[width=0.31\linewidth]{figure/7l11.png}
\label{fig:7l11}}
\subfigure[Example of 3eml, -13.2 kcal/mol]{
\includegraphics[width=0.31\linewidth]{figure/3eml.png}
\label{fig:3eml}}
\subfigure[TOP-100 vs \# oracle call]{
\includegraphics[width=0.42\linewidth]{figure/all_top100.png}
\label{fig:randomwalk1}}
% \subfigure[TOP-10 vs \# oracle call]{
% \includegraphics[width=0.4\linewidth]{figure/all_top10.png}
% \label{fig:randomwalk2}}
\subfigure[Score bar for different runs]{
\includegraphics[width=0.42\linewidth]{figure/sns.png}
\label{fig:randomwalk2}}
% \subfigure[1K oracle call]{
% \includegraphics[width=0.31\linewidth]{figure/errorbar_1k.png}
% \label{fig:randomwalk3}}
\caption{
(a) and (b): Example of ligand poses (generated by \mname) and binding sites of target structures. Example of 7l11: the PDB ID of target is 7l11, which is SARS-COV-2(2019-NCOV) main protease, the Vina score is -10.8 kcal/mol.  
Example of 3eml: the PDB ID is 3eml, which is a human A2A Adenosine receptor, the Vina score is -13.2 kcal/mol.  
(c) and (d): studies of suppressed random-walk behavior. (c) reports TOP-100 docking score as a function of oracle calls. The results are the means and standard deviations of 5 independent runs. (d) shows the bars of TOP-100 docking score for various independent runs. 
}
\label{fig:multiple_run}
\end{figure}

% \begin{figure}[h!]
% \centering
% \subfigure{
% \includegraphics[width=0.86\linewidth]{figure/3eml_example.png}}
% % \subfigure{
% % \includegraphics[width=4.5cm]{figure/3eml_1.png}}
% \caption{Examples of ligand poses (generated by \mname) and binding sites of target structures. The PDB ID of the target is ``3eml''. We observe that the generated molecules have high binding affinity with the designated target. 
% }
% \label{fig:demo}
% \end{figure}












==> NeurIPS 2022 RGA arxiv/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> NeurIPS 2022 RGA arxiv/method.tex <==
\section{Method}
\label{sec:method}


% \subsection{Problem Formulation: Structure-based Drug Design}
% \label{sec:problem}



% Drug design aims to generate novel chemical compounds with desired pharmaceutical properties. 
% Ideally, the generated molecules should be tested in the wet lab for the desired property. 
% In practice, due to cost of wet lab experiment, a computational proxy is usually used. 
% For example, most of the existing machine learning methods focus on optimizing heuristic oracles, such as quantitative estimate of drug-likeness (QED) and  Octanol-water partition coefficient (LogP)~\cite{jin2018learning,You2018-xh,zhou2019optimization,nigam2019augmenting,jin2019learning,korovina2020chembo,jin2020multi,xie2021mars}.
% However, these oracles are too simplistic and do not reflect the complexity of
% real drug discovery problems~\cite{coley2020autonomous,cieplinski2020we}. 

% an experimental evaluation, such as a bioassay, or a high-fidelity simulation, 
% is more difficult to optimize, much more computationally costly and more realistic in drug discovery process~\cite{lyu2019ultra,cieplinski2020we,luo20213d,li2021structure,steinmann2021using}. 
% that require a more data-efficient strategy. 

% In this paper, we focus on structure-based drug design.
% % , which is a more realistic proxy in the context of drug design~\cite{lyu2019ultra,cieplinski2020we,luo20213d,li2021structure,steinmann2021using}.
% The goal is to design drug candidates molecules (a.k.a. ligands) that could bind tight with the disease-related proteins (a.k.a. targets). 
% % The target structure is usually a protein related to the disease. 
% Given the 3D target structure including binding sites,
% % and the binding pocket size and the 3D geometric shape, 
% docking is a popular computational method for assessing the binding affinity, which can be roughly retrieve as the free energy changes during the binding processes. 

In this paper, we focus on structure-based drug design. The goal is to design drug molecules (a.k.a. ligands) that could bind tightly with the disease-related proteins (a.k.a. targets). Given the 3D structures of the target proteins, including binding site information, docking is a popular computational method for assessing the binding affinity, which can be roughly retrieved as the free energy changes during the binding processes. 
We present a variant of genetic algorithm that is guided by reinforcement learning and a docking oracle.
Next, we will first describe the general evolutionary process used in genetic algorithms (Section~\ref{sec:ga}); Then we will present how to model this evolutionary process as a Markov decision process (MDP) where RL framework can be constructed (Section~\ref{sec:mdp}); After that, we describe the detailed implementation of this MDP framework using multiple policy networks (Section~\ref{sec:policy_net}).

% \noindent\textbf{Docking simulation}. 
% The purpose of target-ligand docking is to find the optimal binding between a small molecule (ligand) and a target (target protein). 
% Docking can be conducted using well-commercialized software, such as AutoDock Vina~\cite{trott2010autodock}. The input is a 2D molecular graph, the 3D geometric shape of target and the corresponding binding site. The output is the 3D pose and relative position of the ligand (binds to target) that corresponds to the best binding affinity score. 
% In this paper, we use $X$ to denote the ligand (including its 3D pose that binds to the target), $\calT$ to denote 3D target structures. The mathematical notation table is available in Appendix. 
% In this paper, we leverage one 3D pose and relative coordinates of the ligand that corresponds to the best binding affinity score. 






\subsection{Evolutionary Process}
\label{sec:ga}

In this section, we introduce the primary setting of the evolutionary processes. With both optimization performance and synthetic accessibility taken into account~\cite{gao2020synthesizability,huang2021therapeutics}, we follow the action settings in Autogrow 4.0~\cite{spiegel2020autogrow4}. It demonstrated superior performance over other GA variants in the empirical validation of structure-based drug design~\cite{spiegel2020autogrow4}, and its mutation actions originated from chemical reactions so that the designed molecules are more likely to be synthesizable.
Specifically, an evolutionary processes starts by randomly sampling a \textit{population} of drug candidates from a library. In each \textit{generation} (iteration), it carries out (i) \textit{crossover} between parents selected from the last generation, and (ii) \textit{mutation} on a single child to obtain the offspring pool. An illustration of both crossover and mutation operations is available in Appendix. Note that we only adopted the action settings from Autogrow 4.0, without using other tricks such as elitism.


% an illustration, whose superiority over other GA variants is empirically validated in structure-based drug design~\cite{spiegel2020autogrow4}. 

% Specifically, GA starts from a \textit{population} of molecule candidates. In each \textit{generation} (iteration), it carries out (I) \textit{mutation} and (II) \textit{crossover} to obtain the offspring, as illustrated in Figure~\ref{fig:ga}. 



\noindent\textbf{Crossover}, also called recombination, combines the structure of two parents to generate new children. Following Autogrow 4.0~\cite{spiegel2020autogrow4}, we select two parents from the last generation and search for the largest common substructure shared between them. Then we generate two children by randomly switching their decorating moieties, i.e., the side chains attached to the common substructure. 

\noindent\textbf{Mutation} operates on a single parent molecule and modifies its structure slightly. Following Autogrow 4.0~\cite{spiegel2020autogrow4}, we adopt transformations based on chemical reactions. Unlike naively defined atom-editing actions, mutation steps based on chemical reactions could ensure all modification is reasonable in reality, leading to a larger probability of designing synthesizable molecules.
We included two types of chemical reactions: uni-molecular reactions, which only require one reactant, and bi-molecular reactions, which require two reactants. While uni-molecular reactions could be directly applied to the parent, we sample a purchasable compound to react with the parent when conducting a bi-molecular reaction. In both cases, the parent serves as one reactant, and we use the main product as the child molecule. 
We use the chemical reactions from \cite{spiegel2020autogrow4}, which was originally from \cite{durrant2013autogrow,hartenfeller2011collection}.


\noindent\textbf{Evolution}. At the $t$-th generation (iteration), given a population of molecules denoted as $\mathcal{S}^{(t)}$, we generate an offspring pool denoted as $\mathcal{Q}^{(t)}$ by applying crossover and mutation operations. Then we filter out the ones with undesirable physical and chemical properties (e.g., poor solubility, high toxicity) in the offspring pool and select the most promising $K$ to form the next generation pool ($\mathcal{S}^{(t+1)}$). 



% , offspring are generated by cloning an existing solution; two parents are randomly selected from the population of the last generation. 
% In this paper, following Autogrow 4.0~\cite{spiegel2020autogrow4}, crossover operator finds the largest common substructure that the two parent compounds share and generates a child by randomly combining their decorating moieties. 

% \noindent\textbf{Mutation} operator performs an \textit{in silico} chemical reaction to generate an altered child compound (i.e., product in the chemical reaction) derived from a parent (reactant in the chemical reaction). The chemical reaction here contains two reactants, one is parent molecule, another is from reaction set. 
% The reaction set $\mathcal{R}$ is generated via merging two public reaction libraries: (1) the AutoClickChemRxn set (36 reactions)~\cite{durrant2013autogrow} and (2) RobustRxn set (58 reactions~\cite{hartenfeller2011collection}). 
% Each reaction $\xi$ in reaction set $\mathcal{R}$ contains a SMARTS string based reaction template and a reactant. 
% It uses SMARTS reaction template, together with RDKit~\cite{landrum2006rdkit}, to perform chemical mutations efficiently. 
% The process is written as $X^{\text{parent}}_{\text{mutation}} \xrightarrow[]{\text{mutated by}\ \xi} X^{\text{child}}_{\text{mutation}}$, where $\xi$ is selected reaction (with a reaction template and another reactant).
% The ligand to be mutated and the reaction used for mutation are both randomly selected from previous generation and reaction set $\mathcal{R}$, respectively. 
% Compared with the mutation operator in conventional GA that randomly flipping an arbitrary bit, the reaction-based mutation enhance synthesizability of the generated molecules~\cite{spiegel2020autogrow4}. 


% At the the $t$-th generation (iteration), given a population of molecules, denoted as $\mathcal{S}^{(t)}$, based on crossover and mutation operations, GA generates a bunch of offspring (the set is denoted as $\mathcal{Q}^{(t+1)}$) and select the most promising $K$ ($K$ molecules with best objectives) as the population for the next generation (denoted as $\mathcal{S}^{(t+1)}$). 


\begin{figure}[t]
\centering
\vspace{-15pt}
% \subfigure{\includegraphics[width=0.44\linewidth]{figure/ga_pipeline2.png}}
% \subfigure{\includegraphics[width=0.55\linewidth]{figure/pipeline.png}}
\includegraphics[width=0.86\linewidth]{figure/RGA.png}
\caption{
We illustrate one generation (iteration) of GA (top) and \mname pipeline (bottom). 
Specifically, we train policy networks that take the target and ligand as input to make informed choices on parents and mutation types in \mname.  
}
\vspace{-10pt}
\label{fig:pipeline}
\end{figure}


\subsection{Evolutionary Markov Decision Process}
\label{sec:mdp}

Next we propose the evolutionary Markov decision process (EMDP) that formulates an evolutionary process of genetic algorithm as a Markov decision process (MDP). The primary purpose is to utilize reinforcement learning algorithms to train networks to inform the decision steps to replace random selections. Taking a generation as a state, Markov property that requires $P(\mathcal{S}^{(t+1)} | \mathcal{S}^{(1)}, \cdots, \mathcal{S}^{(t)}) = P(\mathcal{S}^{(t+1)} | \mathcal{S}^{(t)}) $ is naturally satisfied by the evolutionary process described above, where $\mathcal{S}^{(t)}$ denotes the state at the $t$-th generation, which is the population of ligands. We use $X$ to denote a ligand. 
We elaborate essential components for Markov decision process as follows, and the EMDP pipeline is illustrated in Figure~\ref{fig:pipeline}. 

\noindent\textbf{State Space}. We define the population at the $t$-step generation, $\mathcal{S}^{(t)}$, in the evolutionary process as the state at the $t$-step in an EMDP. A state includes population of candidate molecules (i.e., ligand, denoted $X$) and their 3D poses docked to the target, fully observable to the RL agent. At the beginning of the EMDP, we randomly select a population of candidate molecules and use docking simulation to yield their 3D poses as the initial state. 

% In this section, we formulate the generation process of genetic algorithm as a Markov decision process (MDP), which requires that the state transition satisfies the Markov property: $P(\mathcal{S}^{(t+1)} | \mathcal{S}^{(1)}, \cdots, \mathcal{S}^{(t)}) = P(\mathcal{S}^{(t+1)} | \mathcal{S}^{(t)}) $, where $\mathcal{S}^{(t)}$ denotes the state at the $t$-th generation. 
% Markov property is naturally satisfied for GA described above. 
% % Figure~\ref{fig:framework} illustrates a generation process xxxxx
% Then we elaborate four essential components for Markov decision process as follows.  

% \noindent\textbf{State Space}. We define the state $\mathcal{S}^{(t)}$ at the $t$-step generation as the population of candidates and corresponding 3D poses with regard to the target, which is fully observable (by the RL agent). At the beginning of the generation, we randomly select a population of candidate molecules and use docking simulation to yield their 3D poses as the initial state. 


\noindent\textbf{Action Space}. The actions in an EMDP are to conduct the two evolutionary steps: crossover and mutation, in a population. For each evolutionary step, we need two actions to conduct it. Concretely, crossover ($X^{\text{parent 1}}_{\text{crossover}}, X^{\text{parent 2}}_{\text{crossover}} \xrightarrow[]{\text{crossover}} X^{\text{child 1}}_{\text{crossover}}, X^{\text{child 2}}_{\text{crossover}}$) can be divided to two steps:
% \begin{enumerate}
%  \item 
(1) select the first candidate ligand $X^{\text{parent 1}}_{\text{crossover}}$ from the current state (population $\mathcal{S}^{(t)}$);
%  \item 
(2) conditioned on the first selected candidate $X^{\text{parent 1}}_{\text{crossover}}$, select the second candidate ligand $X^{\text{parent 2}}_{\text{crossover}}$ from the remaining candidate ligand set $\calS^{(t)} - \{X^{\text{parent 1}}_{\text{crossover}} \}$ and apply crossover (Section~\ref{sec:ga}) to them. 
% \end{enumerate}

Mutation ($X^{\text{parent}}_{\text{mutation}} \xrightarrow[]{\text{mutated by}\ \xi} X^{\text{child}}_{\text{mutation}}$) can be divided to two steps:
% \begin{enumerate}
%  \item 
(1) select the candidate ligand $X^{\text{parent}}_{\text{mutated}}$ to be mutated from the current state (population $\mathcal{S}^{(t)}$); 
%  \item 
(2) conditioned on the selected candidate ligand $X^{\text{parent}}_{\text{mutated}}$, select the reaction $\xi$ from the reaction set $\mathcal{R}$ and apply it to $X^{\text{parent}}_{\text{mutated}}$. 
% \end{enumerate}

As applying the crossover and mutation steps are deterministic, the actions in an EMDP focus on selecting parents and mutation types. Upon finish the action, we could obtain offspring pool, $\mathcal{Q}^{(t)}$.

\noindent\textbf{State Transition Dynamics}. 
The state transition in an EMDP is identical to the evolution in an evolutionary process. Once we finish the actions and obtain the offspring pool, $\mathcal{Q}^{(t)}=\{X^{\text{child 1}}_{\text{}}, X^{\text{child 2}}_{\text{}}, \cdots \}$, we apply molecular quality filters to filter out the ones unlikely to be drug and then select the most promising $K$ to form the parent set for the next generation ($\mathcal{S}^{(t+1)}$). 

\noindent\textbf{Reward}. We define the reward as the binding affinity change (docking score). The actions leading to stronger binding score would be prioritized. As there is no ``episode'' concept in an EMDP, we treat every step equally.%, i.e., no intermediate and final reward.

% \noindent\textbf{Action Space}. We define two actions for both mutation and crossover operations. Mutation has two actions:
% \begin{enumerate}
%  \item select the candidate ligand $X^{\text{parent}}_{\text{mutated}}$ to be mutated from the current state (population $\mathcal{S}^{(t)}$); 
%  \item conditioned on the selected candidate ligand $X^{\text{parent}}_{\text{mutated}}$, select the reaction $\xi$ from the reaction set $\mathcal{R}$ to mutate. 
% \end{enumerate}
% Crossover operation also has two actions:
% \begin{enumerate}
%  \item select the first candidate ligand $X^{\text{parent 1}}_{\text{crossover}}$ from the current state (population $\mathcal{S}^{(t)}$);
%  \item conditioned on the first selected candidate $X^{\text{parent 1}}_{\text{crossover}}$, select the second candidate ligand $X^{\text{parent 2}}_{\text{crossover}}$ from the remaining candidate ligand set $\calS^{(t)} - \{X^{\text{parent 1}}_{\text{crossover}} \}$. 
% \end{enumerate}

% $\mathcal{Q}^{(t)}$

% \noindent\textbf{State Transition Dynamics}. 
% Once a valid action is selected, the state transition is deterministic. Specifically, the mutation process is denoted $X^{\text{parent}}_{\text{mutation}} \xrightarrow[]{\text{mutated by}\ \xi} X^{\text{child}}_{\text{mutation}}$, where $\xi$ is selected reaction (with a reaction template and another reactant). The crossover process is denoted $X^{\text{parent 1}}_{\text{crossover}}, X^{\text{parent 2}}_{\text{crossover}} \xrightarrow[]{\text{crossover}} X^{\text{child 1}}_{\text{crossover}}, X^{\text{child 2}}_{\text{crossover}}$. 
% We draw multiple samples from action space to generate multiple offspring ($X^{\text{child}}_{\text{}}$), infeasible actions that do not return a valid offspring molecule are filtered out. After generating all the offspring, we keep the best K offspring in the population for the next generation (i.e., $\mathcal{S}^{(t+1)}$). 


% \noindent\textbf{Reward}. Intermediate reward is the improvement of binding affinity (docking score) and are used to guide the behaviour of the RL agent (policy neural network below). 
% In Structure-based drug design, the reward is the binding affinity between the ligand and the target. 

% The MDP pipeline is illustrated in Figure~\ref{fig:pipeline}. 



\subsection{Target-Ligand Policy Network}
\label{sec:policy_net}

To utilize molecular structures' translational and rotational invariance, we adopt equivariance neural networks (ENNs)~\cite{satorras2021n} as the target-ligand policy neural networks to select the actions in both mutation and crossover steps. Each ligand has a 3D pose that binds to the target protein, and the complex serves as the input of ENN.


% We design target-ligand policy neural networks to select the actions in both mutation and crossover operations. Each ligand has 3D pose that binds to the 3D target structure. We use an equivariance neural network (ENN)~\cite{satorras2021n} to model the 3D geometric shape of target/ligand/target-ligand complex to learn the selection probability of the ligand. 
% The equivariance neural network achieves state-of-the-art performance in modeling 3D geometric molecule data~\cite{townshend2021atom3d} and is translation- and rotation- invariant with regard to the 3D graph. That is, the translation and rotation on the 3D graph (coordinates) would not change ENN's output. 

Specifically, we want to model a 3D graph $\calY$, which can be ligand, target, or target-ligand complex. The input feature can be described as $\calY = (\calA, \calZ)$, where $\calA$ represents atoms' categories (the vocabulary set $\calV =\{H, C, O, N, \cdots\}$) and $\calZ$ represents 3D coordinates of the atoms. 
Suppose $\bfD \in \RB^{|\calV|\times d}$ is the embedding matrix of all the categories of atoms in a vocabulary set $\calV$, is randomly initialized and learnable, $d$ is the hidden dimension in ENN. 
Each kind of atom corresponds to a row in $\bfD$. 
We suppose there are $N$ atoms, and each atom corresponds to a node in the 3D graph. 
Node embeddings at the $l$-th layer are denoted as $\bfH^{(l)} = \{\bfh^{(l)}_i\}_{i=1}^{N}$, where $l=0,1,\cdots,L$, $L$ is number of layers in ENN. 
The initial node embedding $\bfh_i^{(0)} = \bfD^\top {\bfa_i} \in \RB^{d}$ embeds the $i$-th node, where ${\bfa_i}$ is one-hot vector that encode the category of the $i$-th atom.  
Coordinate embeddings at the $l$-th layer are denoted $\bfZ^{(l)} = \{\bfz_i^{(l)}\}_{i=1}^{N}$. 
The initial coordinate embeddings $\bfZ^{(0)} = \{\bfz_i^{}\}_{i=1}^{N}$ are the real 3D coordinates of all the nodes.  
The following equation defines the feedforward rules of ENN, for $i,j=1,\cdots,N, \ i\neq j,\ l=0,1,\cdots,L-1$, we have 
\begin{equation}
\label{eqn:ENN}
\begin{aligned}
& \bfw^{(l+1)}_{ij} = \text{MLP}_{e} \Big( \bfh^{(l)}_i \oplus \bfh^{(l)}_j \oplus || \bfz_i^{(l)} - \bfz_j^{(l)} ||_2^2 \Big) \ \   \in \RB^{d}, 
% \\
& \bfv^{(l+1)}_i = \sum_{j=1,j\neq i}^{N} \bfw^{(l+1)}_{ij} \ \  \in \RB^{d}, \\
& \bfz_i^{(l+1)} = \bfz_i^{(l)} + \sum_{j=1,j\neq i}^{N} \Big(\bfz_i^{(l)} - \bfz_j^{(l)} \Big) \text{MLP}_{x} \Big(\bfw^{(l)}_{ij} \Big) \in \RB^{3}, 
% \\
& \bfh^{(l+1)}_i = \text{MLP}_h \Big(\bfh_i^{(l)} \oplus \bfv^{(l+1)}_i \Big) \in \RB^{d}, \\
& \bfh_{\calY} = \sum_{i=1}^{N} \bfh_{i}^{(L)} \ \in \RB^{d} \ \ \ \  \ \ \implies \underline{\bfh_{\calY} = \text{ENN}(\calY)}
\end{aligned}
\end{equation}
where $\oplus$ denotes the concatenation of vectors; $\text{MLP}_{e}(\cdot): \RB^{2d+1}\xrightarrow[]{}\RB^{d}; 
\text{MLP}_{x}(\cdot): \RB^{d}\xrightarrow[]{}\RB; 
\text{MLP}_{h}(\cdot): \RB^{2d}\xrightarrow[]{}\RB^{d}$ are all two-layer multiple layer perceptrons (MLPs) with Swish activation in the hidden layer \cite{ramachandran2017searching}. 
At the $l$-th layer, $\bfw^{(l)}_{ij}$ represents the message vector for the edge from node $i$ to node $j$; $\bfv^{(l)}_{i}$ represents the message vector for node $i$, $\bfz^{(l)}_i$ is the position embedding for node $i$; $\bfh_i^{(l)}$ is the node embedding for node $i$. 
$\bfH^{(L)} = [\bfh_1^{(L)}, \cdots, \bfh_N^{(L)}]$ are the node embeddings of the $L$-th (last) layer. 
We aggregate them using sum function as readout function to obtain a representation of the 3D graph, denoted $\bfh_{\calY}$. The whole process is written as $\bfh_{\calY} = \text{ENN}(\calY)$.



\noindent\textbf{Crossover Policy Network}. 
We design two policy networks for two corresponding actions in a crossover, as mentioned in Section~\ref{sec:mdp}. 
(1) the first action in crossover operation is to select the first parent ligand $X^{\text{parent 1}}_{\text{crossover}}$ from the population $\mathcal{S}^{(t)}$. 
Similar to the first action in mutation operation, we obtain a valid probability distribution over all the available ligands based on target-ligand complex as input feature and ENN as the neural network architecture, the selection probability of the ligand $X^{\text{parent 1}}_{\text{crossover}} \in \calS^{(t)} $ is  $p_{\text{crossover}}^{(1)}(X^{\text{parent 1}}_{\text{crossover}} | \calS^{(t)}) = \frac{\exp{\big( \text{MLP} (\bfh_{\calT \& X^{\text{parent 1}}_{\text{crossover}}} )\big)}}{\sum_{X'\in \calS^{(t)}} \exp{\big( \text{MLP}(\bfh_{\calT\& X'})\big)}}$, where $\calT$ and $X$ denotes target and ligand (including 3D pose), respectively, $\calT \& X$ denotes target-ligand complex. 
% It corresponds to the policy network in Figure~\ref{fig:pipeline}. 
(2) The second action is to select the second parent ligand conditioned on the first parent ligand selected in the first action. 
Specifically, for ligand in the remaining population set, we concatenate the ENN's embedding of the target, first parent ligand $X^{\text{parent 1}}_{\text{crossover}}$ and the second parent ligand \marked{$X^{\text{parent 2}}_{\text{mutation}}$}, and feed it into an MLP to estimate a scalar as an unnormalized probability. 
The unnormalized probabilities for all the ligands in the remaining population set are normalized via softmax function, i.e., 
$p_{\text{crossover}}^{(2)}(X^{\text{parent 2}}_{\text{crossover}} | X^{\text{parent 1}}_{\text{crossover}}, \mathcal{S}^{(t)} ) = \text{Softmax} \big\{\text{MLP}(\bfh_{\calT}\oplus \bfh_{X^{\text{parent 1}}_{\text{crossover}}} \oplus \bfh_{X^{\text{parent 2}}_{\text{crossover}}}), \cdots, \big\}_{X^{\text{parent 2}}_{\text{crossover}} \in \calS^{(t)}-\{X^{\text{parent 1}}_{\text{crossover}}\} }$. 
% It corresponds to the ``crossover policy network 2'' in Figure~\ref{fig:pipeline}. 
Given two parents ligands, crossover finds the largest substructure that the two parent compounds share and generates a child by combining their decorating moieties. Thus, the generation of child ligands are deterministic, and the probability of the generated ligands $X^{\text{child}}_{\text{crossover}}$ is 
\begin{equation}
\label{eqn:crossover_prob}
\begin{aligned}
& p_{\text{crossover}}(X_{\text{crossover}}^{\text{child 1}}, X_{\text{crossover}}^{\text{child 2}} | \mathcal{S}^{(t)}) 
= p_{\text{crossover}}(X_{\text{crossover}}^{\text{parent 1}}, X_{\text{crossover}}^{\text{parent 2}} | \mathcal{S}^{(t)}) \\ 
=\ & p_{\text{crossover}}^{(1)}(X^{\text{parent 1}}_{\text{crossover}} | \mathcal{S}^{(t)})
\cdot 
p_{\text{crossover}}^{(2)}(X^{\text{parent 2}}_{\text{crossover}} | X^{\text{parent 1}}_{\text{crossover}}, \mathcal{S}^{(t)} ). 
\end{aligned}
\end{equation}


\noindent\textbf{Mutation Policy Network}. We design two policy networks for two corresponding actions in mutation, as mentioned in Section~\ref{sec:mdp}. 
(1) the first action in mutation operation is to select a candidate ligand to be mutated from population $\mathcal{S}^{(t)}$. It models the 3D target-ligand complex to learn if there is improvement space in the current complex. 
Formally, we obtain a valid probability distribution over all the available ligands based on target-ligand complex as input feature and ENN as neural architecture, the selection probability of the ligand $X^{\text{parent}}_{\text{mutation}} \in \calS^{(t)} $ is  $p_{\text{mutation}}^{(1)}(X^{\text{parent}}_{\text{mutation}} | \calS^{(t)}) = \frac{\exp{\big( \text{MLP}( \bfh_{\calT \& X^{\text{parent}}_{\text{mutation}}} ) \big)}}{\sum_{X'\in \calS^{(t)}} \exp{\big(  \text{MLP}( \bfh_{\calT\& X'}) \big)}}$, where $\calT \& X$ denotes target-ligand complex, $\bfh_{\calT \& X} = \text{ENN}(\calT \& X)$ represents the ENN's embedding of target-ligand complex. 
(2) The second action is to select the SMARTS reaction from the reaction set conditioned on the selected ligand in the first action. Specifically, for each reaction, we generate the new ligand $X^{\text{child}}_{\text{mutation}}$, then obtain the embedding of target, first ligand $X^{\text{parent}}_{\text{mutation}}$ and the new ligand $X^{\text{child}}_{\text{mutation}}$ through ENN, concatenate these three embeddings and feed it into \marked{an} MLP to estimate a scalar as unnormalized probability. 
The unnormalized probabilities for all the reactions are normalized via softmax function, i.e.,  
$p_{\text{mutation}}^{(2)}(\xi | X^{\text{parent}}_{\text{mutation}}, \calS^{(t)}) = \text{Softmax} \big\{\text{MLP}(\bfh_{\calT} \oplus \bfh_{X^{\text{parent}}_{\text{mutation}}} \oplus \bfh_{X^{\text{child}}_{\text{mutation}}} ]), \cdots, \big\}_{\xi \in \mathcal{R}}^{}$, where $X^{\text{parent}}_{\text{mutation}} \xrightarrow[]{\text{mutated by}\ \xi} X^{\text{child}}_{\text{mutation}}$, $\calR$ is the reaction set. 
The probability of the generated ligand $X^{\text{child}}_{\text{mutation}}$ is 
\begin{equation}
\label{eqn:mutation_prob}
p_{\text{mutation}}(X^{\text{child}}_{\text{mutation}} | \mathcal{S}^{(t)}) = p_{\text{mutation}}^{(1)}(X^{\text{parent}}_{\text{mutation}} | \calS^{(t)}) \cdot 
p_{\text{mutation}}^{(2)}(\xi | X^{\text{parent}}_{\text{mutation}}, \calS^{(t)}). 
\end{equation}


\noindent\textbf{Policy Gradient}. 
We leverage policy gradient to train the target-ligand policy neural network. Specifically, we consider maximizing the expected reward as objective via REINFORCE~\cite{Olivecrona}, 
\begin{equation}
\label{eqn:policy}
\max\ \EB_{X \sim p(X | \mathcal{S}^{(t)})}\big[ \text{Reward}(X) \big], 
\end{equation}
where $p(X)$ is defined in Equation~\eqref{eqn:crossover_prob} and~\eqref{eqn:mutation_prob} for crossover and mutation, respectively. 
The whole pipeline is illustrated in Figure~\ref{fig:pipeline}. 
To provide a warm start and leverage the structural information, we pretrain the ENNs on 3D target-ligand binding affinity prediction task, where the inputs are the target-ligand complexes, and the outputs are their binding affinity. 


% \noindent\textbf{Policy Gradient}. 
% We leverage policy gradient to train the target-ligand policy neural network. 
% Specifically, we consider maximizing the expected reward as objective via REINFORCE~\cite{Olivecrona}, 
% \begin{equation}
% \label{eqn:policy}
% \max\ \EB_{X \sim p(X | \mathcal{S}^{(t)})}\big[ \text{Reward}(X) \big], 
% \end{equation}
% where $p(X)$ is defined in Equation~\eqref{eqn:crossover_prob} and~\eqref{eqn:mutation_prob} for crossover and mutation mutation, respectively. 
% The reward is the binding affinity between the ligand and the target. Larger reward value are desirable. 
% Each episode corresponds to a generation in \mname and we decompose the whole reward into the sum of multiple intermediate reward in multiple generations. 
% The intermediate reward is the improvement of binding affinity over the last generation.  
% The whole pipeline is illustrated in Figure~\ref{fig:pipeline}. 
% % \noindent\textbf{Pretraining}. 
% To provide a warm start, we pretrain ENN on 3D target-ligand binding affinity prediction task, where the input are the target-ligand complex and the output is their binding affinity.  
% \noindent\textbf{Summarization}. 






==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

